Opaque Contracts

Firms have access to abundant data on market participants. They use these data to target contracts to agents with specific characteristics, and describe these contracts in opaque terms. In response to such practices, recent proposed regulations aim to increase transparency, especially in digital markets. In order to understand when opacity arises in contracting and the potential effects of proposed regulations, we study a moral hazard model in which a risk-neutral principal faces a continuum of weakly risk-averse agents. The agents differ in an observable characteristic that affects the payoff of the principal. In a described contract, the principal sorts the agents into groups, and to each group communicates a distribution of output-contingent payments. Within each group, the realized distribution of payments must be consistent with the communicated contract. A described contract is transparent if the principal communicates the realized contract to the agent ex-ante, and otherwise it is opaque. We provide a geometric characterization of the principal's optimal described contract as well as conditions under which the optimal described mechanism is transparent and opaque. We apply our results to the design and description of driver payment schemes on ride-hailing platforms.

==> IDs_tikz.tex <==

\begin{tikzpicture}
\tikzset{%
  every node/.style={line width=.35mm},
  every edge/.style={line width=.35mm}
}
% Circles
\node[draw, diamond, minimum size=7mm, label=center:$u$] at (0,0) (u) {};
\node[draw, circle, minimum size=7mm, label=center:$x$] at (0,-15mm) (x) {};
\node[draw, circle, minimum size=7mm, label=center:$q$] at (0,-30mm) (q) {};

% Square
\node[draw, minimum size=7mm, label=center:$a_k$] at (-20mm, -30mm) (a) {};
\node[label=center:\textbf{(*)}] at (-10mm, -38mm) (*) {};

% Arrows
\draw[dotted,thick, ->] (q) -- (x) node[midway, left] {$g_k$};
\draw[thick,->] (x) -- (u);
\draw[thick,->] (a) -- (u);
\draw[thick,->] (a) -- (q);

\end{tikzpicture} \hspace{10mm} \begin{tikzpicture}
\tikzset{%
  every node/.style={line width=.35mm},
  every edge/.style={line width=.35mm}
}
% Circles
\node[draw, diamond, minimum size=7mm, label=center:$u$] at (0,0) (u) {};
\node[draw, circle, minimum size=7mm, label=center:$x$] at (0,-15mm) (x) {};
\node[draw, circle, minimum size=7mm, label=center:$q$] at (0,-30mm) (q) {};


% Square
\node[draw, minimum size=7mm, label=center:$a$] at (-20mm, -30mm) (a) {};
\node[label=center:\textbf{(**)}] at (-10mm, -38mm) (*) {};


% New circles
\node[draw, circle, minimum size=7mm, label=center:$m$] at (-20mm, -15mm) (m) {};
\node[draw, circle, minimum size=7mm, label=center:$s$] at (-20mm, 0) (s) {};


% Arrows
\draw[dotted, thick, ->] (q) -- (x) node[midway, left] {$\psi$};
\draw[dotted, thick, ->] (m) -- (x) node[midway, above] {$\psi$};
\draw[dotted, thick, ->] (s) -- (x) node[midway, above] {$\psi$};
\draw[dotted, thick, ->] (s) -- (m) node[midway, left] {$\omega$};
\draw[thick,->] (x) -- (u);
\draw[thick,->] (m) -- (a);
\draw[thick,->] (a) -- (u);
\draw[thick,->] (a) -- (q);

\end{tikzpicture}

==> mycommands.tex <==
%% ITEMIZE & ENUMERATE ENVIRONMENTS W/O BIG PARAGRAPH SKIPS
\usepackage{accents}
\usepackage{enumitem}


\newenvironment{itemize*}%
  {\begin{itemize}%
    \setlength{\itemsep}{0pt}%
    \setlength{\parskip}{0pt}}%
  {\end{itemize}}
  
  \newenvironment{myquote}{%%
  \begin{itemize}[topsep=0pt]
  \item[]}{\end{itemize}}

\newenvironment{enumerate*}%
  {\begin{enumerate}%
    \setlength{\itemsep}{0pt}%
    \setlength{\parskip}{0pt}}%
  {\end{enumerate}}

\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}

\usepackage{subcaption}

\usepackage[round]{natbib}
\bibliographystyle{aer}
\usepackage{sectsty} % For section format.
%% SECTION STUFF 
\sectionfont{\fontsize{13}{13}\selectfont}
\subsectionfont{\fontsize{11}{11}\selectfont}
\renewcommand{\thesection}{\arabic{section}}
\renewcommand{\thesubsection}{\arabic{section}.\arabic{subsection}}

% USEFUL SYMBOLS
\renewcommand{\P}{\mathbb{P}}
\newcommand{\br}{\mathbf{br}}
\newcommand{\Pj}{\mathbb{P}_j}
\newcommand{\E}{\mathbb{E}}
\newcommand{\ee}{\mathcal{E}}
\newcommand{\yy}{\mathcal{Y}}
\newcommand{\I}{\mathcal{I}}
\newcommand{\thetahat}{\hat{\theta}}
\newcommand{\F}{\mathbf{F}}
\newcommand{\Gsp}{G^{SP}}
\newcommand{\starc}{\textbf{(*)}}
\newcommand{\myline}{\begin{center}\noindent\rule{8cm}{0.4pt}\end{center}}
\newcommand{\Var}{\mathbb{V}\text{ar}}
\newcommand{\Cov}{\text{Cov}}
\newcommand{\ubar}[1]{\underaccent{\bar}{#1}}
%\newcommand{\ubar}[1]{\underline{#1}
\newcommand{\thetalow}{\ubar{\theta}}
\newcommand{\thetahi}{\bar{\theta}}
\newcommand{\nulow}{\ubar{\nu}}
\newcommand{\nuhi}{\bar{\nu}}
\newcommand{\ind}{\mathbf{1}}
\newcommand{\what}{\textcolor{red}{\textbf{(???)}}}
\newcommand{\Ytilde}{\tilde{Y}}
\newcommand{\ctilde}{\tilde{c}}
\newcommand{\qwf}{q^{wf}}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
\newcommand{\Y}{\mathbf{Y}}
\newcommand{\one}{\mathbf{1}}
\newcommand{\Ww}{\mathcal{W}}
\newcommand{\qmin}{q^{\min}}
\newcommand{\qmax}{q^{\max}}
\newcommand{\N}{\mathcal{N}}
\newcommand{\B}{\mathcal{B}}
\newcommand{\x}{\mathbf{x}}
\newcommand{\y}{\mathbf{y}}
\newcommand{\ybar}{\bar{y}}
\newcommand{\pbar}{\bar{p}}
\newcommand{\Beta}{\operatorname{Beta}}
\newcommand{\qbar}{\bar{q}}
\newcommand{\cbar}{\bar{c}}
\newcommand{\qubar}{\underline{q}}
\newcommand{\nubar}{\bar{\nu}}
\newcommand{\ytilde}{\tilde{y}}
\renewcommand{\v}{\mathbf{v}}
\newcommand{\w}{\mathbf{w}}
\renewcommand{\c}{\mathbf{c}}
\newcommand{\s}{\mathbf{s}}
\newcommand{\ones}{\mathbf{1}}
\renewcommand{\a}{\mathbf{a}}
\renewcommand{\b}{\mathbf{b}}
\newcommand{\g}{\mathbf{g}}
\newcommand{\J}{\mathbf{J}}
\newcommand{\nuhat}{\hat{\nu}}
\newcommand{\A}{\mathbf{A}}
\newcommand{\var}{\operatorname{var}}
\newcommand{\V}{\mathbf{V}}
\newcommand{\WW}{\mathbb{W}}
\newcommand{\bSigma}{\mathbf{\Sigma}}
\newcommand{\G}{\mathbf{G}}
\newcommand{\zero}{\mathbf{0}}
\newcommand{\M}{\mathbf{M}}
\newcommand{\MM}{\mathbf{M}}
\newcommand{\K}{\mathcal{K}}
\newcommand{\X}{\mathbf{X}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\T}{\mathbf{T}}
\newcommand{\Diff}{\operatorname{Diff}}
\renewcommand{\t}{\mathbf{t}}
\newcommand{\ql}{q_L}
\renewcommand{\d}{\text{d}}
\newcommand{\qh}{q_H}
\newcommand{\tl}{t_L}
\newcommand{\barcni}{\bar{c}_{-i}}
\newcommand{\cl}{c_L}
\newcommand{\cn}{c_N}
\newcommand{\bb}{\mathbf{b}}
\renewcommand{\th}{t_H}
\newcommand{\thetah}{\theta_H}
\newcommand{\C}{\mathcal{C}}
\newcommand{\thetal}{\theta_L}
\newcommand{\xtilde}{\tilde{x}}
\newcommand{\bxtilde}{\mathbf{\tilde{x}}}
\newcommand{\grad}{\nabla}
\newcommand{\btheta}{\boldsymbol{\theta}}
\newcommand{\bep}{\boldsymbol{\epsilon}}
\newcommand{\mvpf}{\textsc{mvpf}}
\newcommand{\fe}{\textsc{fe}}
\newcommand{\wtp}{\textsc{wtp}}
\newcommand{\WS}{\operatorname{WS}}
\newcommand{\phat}{\hat{p}}
\newcommand{\vc}{\vec{c}}
\newcommand{\p}{\mathbf{p}}
\newcommand{\D}{\mathcal{D}}
\newcommand{\Q}{\mathcal{Q}}
\newcommand{\SWF}{\operatorname{SWF}}
\newcommand{\default}{\text{default}}
\newcommand{\state}{\text{state }}
\newcommand{\varep}{\varepsilon}
\newcommand{\tildef}{\tilde{f}}



%% ENVIRONMENTS 
\newtheorem{theorem}{Theorem}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{condition}[theorem]{Condition}
\newtheorem{corollary}{Corollary}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{definition}{Definition}
\newtheorem{lemma}{Lemma}
\newtheorem{proposition}{Proposition}
\newtheorem{remark}{Remark}
\newtheorem{solution}[theorem]{Solution}
\newtheorem{assumption}{Assumption}
\renewenvironment{proof}[1][Proof]{\textbf{#1.} }{\ \rule{0.5em}{0.5em}}
\theoremstyle{definition}
\newtheorem{example}{Example}


==> risk_aversion_proof.tex <==
Consider any strictly concave, increasing, agent utility function $u(x)$ and consider the sequence of utility functions $u(\rho x)$, $\rho \ge 1$.
\begin{theorem}
As $\rho \to \infty$, the gains from opacity vanish. In other words, for every $f \in \Delta (S)$
\[
\lim_{\rho \to \infty} \overline{V}(f) = V^T(f).
\]
\end{theorem}
\begin{proof}
Let $f \in \Delta(S)$ and let $(g, \hat g)$ be an optimal coarse contract for population $f$. We will construct a transparent contract that yields vanishingly less utility than the optimal coarse contract as $\rho \to \infty$. 

To do so, for each state $s\in S$, we can adjust the payment in the realized contract $g(q(a),s)$ such that, for each action $a \in A$, the agent is indifferent between the optimal coarse contract $\hat g$ and this modified realized, transparent contract $\tilde g_k(q(a),s)$:
\begin{equation}
\hat g(q(a)) \sim \tilde g_k(s,q(a)).\label{eq:indifference}
\end{equation}
One property of this contract is that the agent will choose the same action $a \in A$ in each of the contracts $\tilde g_k(s,q(a))$ and in the fully coarse contract. We will show that for large enough $\rho$, the additional payments needed to make agents indifferent go to zero. In order for the agent to be indifferent, the addition payment $x$ must satisfy:
\[
u(\rho g(s,q(a^*))+\rho x) = \E[u(\rho \hat g(q(a^*))]
\]
This holds if and only if 
\[
x = u^{-1}(\E[u(\rho \hat g(q(a^*))])/\rho - g(s,q(a^*))
\]

\[
\E_{q}[u(\hat g(q(a^*)) - u(g(s,q(a^*))].      u(g(s,q(a^*))+x) = \E[u(\hat g(q(a^*))]
\]
As $S$ is finite, it is enough to show this for every $s \in S$. Fix $s \in S$. We can view $\hat g(q(a^*))$ as a compound lottery with an member lottery $u(g_k(q(a^*))$. The following lemma is sufficient to prove the claim.
\begin{lemma}
Let $u$ be any strictly concave, positive function function with $\rho \in \R_+$ and let $l$ be any finite compound lottery distribution on $\R$. Then,
\[
\lim_{\rho \to \infty} \sum_{x \in \supp g} g(x) \E[u(\rho x)] \le  \E[u(\rho y)].
\]
for any $y$ that is a member of the lottery $l$.
\end{lemma}
\begin{proof}
This statement is applied by the following, stronger statement: For any lottery $g$
\[
\lim_{\rho \to \infty} \sum_{x \in \supp g} g(x) u(\rho x) \le  u(\rho\min \supp g).
\]
By the intermediate value theorem ...
\end{proof}
\end{proof}
